ORDO: Fine-Grained Motion Understanding in Video LLMs via Order-Dependent Supervision

Video large language models (video LLMs) answer a wide range of questions about real videos, yet they remain weak at fine-grained motion such as whether an object speeds up or slows down. Existing methods train these models on synthetic motion clips, on order pretext tasks such as reordering shuffled clips, or with rewards that compare ordered and perturbed frames. None of them requires that the label be unrecoverable from the frames once their order is discarded, so a model can fit such data from static cues without learning to use frame order. We propose ORDO, a framework that builds this requirement into the training data. We define order-necessary supervision as data in which the unordered set of frames has the same distribution under competing labels, and we realise it for motion attributes with three constructions, time-reversal pairing, matched spatial extent and uniform interval coverage. A procedural curriculum of six motion primitives instantiates these constructions, and low-rank adapters of the language model are trained on it with an answer-level objective and self-distillation replay on real videos. With 4,000 synthetic clips, ORDO raises the mean accuracy over four motion benchmarks by +7.6, +4.9 and +5.1 points on Qwen3.5-9B, Qwen3-VL-8B and Molmo2-8B, while the same training with shuffled frames changes it by less than one point. Code and generator will be made publicly available.

==> tables/tabS_vsdata.tex <==
SynRL data & +5.5\,{\scriptsize[+4.5, +6.5]} & +3.9\,{\scriptsize[+2.9, +4.8]} \\
MoDirect-Inst & +5.6\,{\scriptsize[+4.6, +6.6]} & -- \\
Temporal jigsaw, s0 & +5.2\,{\scriptsize[+4.3, +6.2]} & +2.8\,{\scriptsize[+1.9, +3.7]} \\
Temporal jigsaw, s1 & +4.7\,{\scriptsize[+3.7, +5.6]} & +1.2\,{\scriptsize[+0.3, +2.1]} \\
Arrow of time & +7.8\,{\scriptsize[+6.8, +8.8]} & +4.6\,{\scriptsize[+3.7, +5.6]} \\

